A unified joint reconstruction approach in structured illumination microscopy using unknown speckle patterns

The structured illumination microscopy using unknown speckle patterns has shown the capacity to surpass the Abbe's diffraction barrier, giving the possibility to design cheap and versatile SIM devices. However, the state-of-the-art joint reconstruction methods in this framework has a relatively low contrast in super-resolution part in comparison to conventional SIM and the hyper-parameter is not easy to tune. In this paper, a unified joint reconstruction approach is proposed with the hyper-parameter proportional to the noise level. Different regularization terms could be evaluated under the same model. Moreover, the degradation entailed by out-of-focus light could be solved in speckle illumination setup easily.

==> alphabet.tex <==
% Document LaTeX	Auteur : Guy Le Besnerais	Date : 25/05/94
% Modification : J.-F. Gio	(15/09/95)
%			        J.I. (format Latex 2e, taille adaptative 22/03/99)

% Objet : Definitions compactes d'alphabets pour ecriture en Math
% b pour bold italique : \Ab
% v pour bold droit : \Av
% D pour droit : \AD
% Capitale pour capitale : \Lambda

\typeout{\space}
\typeout{\space\space\space\space Fichier 'alphabet.tex' -- LSS 1994/95/99}
\typeout{\space\space\space\space (necessite les packages xspace et amsmath)}
\typeout{\space}

\RequirePackage{amsmath}
\RequirePackage{xspace}
%\usepackage{amsmath}
%\usepackage{xspace}

%%%% NEW - NEW - %%%%% Small caps gras %%%% 05-06-98 %%%% JFG %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%% Merci \`a Caro %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareFontShape{T1}{cmr}{bx}{sc}{
	 <8> <9> <10> <10.95> dcbsc10
	 <12> <14.4> dcbsc10
	 <17.28> <20.74> <24.88> dcbsc10
	 }{}
% SC en bold (Hack !)
\DeclareFontShape{T1}{cmr}{b}{sc}{
	 <8> <9> <10> <10.95> dcbsc10
	 <12> <14.4> dcbsc10
	 <17.28> <20.74> <24.88> dcbsc10
	 }{}%

\def\scb#1{\bfseries {\scshape #1}}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% DEFINITIONS PRELIMINAIRES 

% definition pour \xspace
\def\XS{\xspace}

% Style gras italique (Necessite amsmath)
\def\sbm#1{\ensuremath{\boldsymbol{#1}}}               

% Style droit en math
\def\sdm#1{\ensuremath{\mathrm{#1}}}

% Style gras droit
\def\sbv#1{\ensuremath{\mathbf{#1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% ALPHABET GRAS ITALIQUE
% Taille adaptative

\def\Ab{{\sbm{A}}\XS}  \def\ab{{\sbm{a}}\XS}
\def\Bb{{\sbm{B}}\XS}  \def\bb{{\sbm{b}}\XS}
\def\Cb{{\sbm{C}}\XS}  \def\cb{{\sbm{c}}\XS}
\def\Db{{\sbm{D}}\XS}  \def\db{{\sbm{d}}\XS}
\def\Eb{{\sbm{E}}\XS}  \def\eb{{\sbm{e}}\XS}
\def\Fb{{\sbm{F}}\XS}  \def\fb{{\sbm{f}}\XS}
\def\Gb{{\sbm{G}}\XS}  \def\gb{{\sbm{g}}\XS}
\def\Hb{{\sbm{H}}\XS}  \def\hb{{\sbm{h}}\XS}
\def\Ib{{\sbm{I}}\XS}  \def\ib{{\sbm{i}}\XS}
\def\Jb{{\sbm{J}}\XS}  \def\jb{{\sbm{j}}\XS}
\def\Kb{{\sbm{K}}\XS}  \def\kb{{\sbm{k}}\XS}
\def\Lb{{\sbm{L}}\XS}  \def\lb{{\sbm{l}}\XS}
\def\Mb{{\sbm{M}}\XS}  \def\mb{{\sbm{m}}\XS}
\def\Nb{{\sbm{N}}\XS}  \def\nb{{\sbm{n}}\XS}
\def\Ob{{\sbm{O}}\XS}  \def\ob{{\sbm{o}}\XS}
\def\Pb{{\sbm{P}}\XS}  \def\pb{{\sbm{p}}\XS}
\def\Qb{{\sbm{Q}}\XS}  \def\qb{{\sbm{q}}\XS}
\def\Rb{{\sbm{R}}\XS}  \def\rb{{\sbm{r}}\XS}
\def\Sb{{\sbm{S}}\XS}  \def\sb{{\sbm{s}}\XS}
\def\Tb{{\sbm{T}}\XS}  \def\tb{{\sbm{t}}\XS}
\def\Ub{{\sbm{U}}\XS}  \def\ub{{\sbm{u}}\XS}
\def\Vb{{\sbm{V}}\XS}  \def\vb{{\sbm{v}}\XS}
\def\Wb{{\sbm{W}}\XS}  \def\wb{{\sbm{w}}\XS}
\def\Xb{{\sbm{X}}\XS}  \def\xb{{\sbm{x}}\XS}
\def\Yb{{\sbm{Y}}\XS}  \def\yb{{\sbm{y}}\XS}
\def\Zb{{\sbm{Z}}\XS}  \def\zb{{\sbm{z}}\XS}

% ALPHABET CURSIF
% Cursif(majuscules), taille adaptative

\def\Ac{{\ensuremath{\mathcal{A}}}\XS}
\def\Bc{{\ensuremath{\mathcal{B}}}\XS}
\def\Cc{{\ensuremath{\mathcal{C}}}\XS}
\def\Dc{{\ensuremath{\mathcal{D}}}\XS}
\def\Ec{{\ensuremath{\mathcal{E}}}\XS}
\def\Fc{{\ensuremath{\mathcal{F}}}\XS}
\def\Gc{{\ensuremath{\mathcal{G}}}\XS}
\def\Hc{{\ensuremath{\mathcal{H}}}\XS}
\def\Ic{{\ensuremath{\mathcal{I}}}\XS}
\def\Jc{{\ensuremath{\mathcal{J}}}\XS}
\def\Kc{{\ensuremath{\mathcal{K}}}\XS}
\def\Lc{{\ensuremath{\mathcal{L}}}\XS}
\def\Mc{{\ensuremath{\mathcal{M}}}\XS}
\def\Nc{{\ensuremath{\mathcal{N}}}\XS}
\def\Oc{{\ensuremath{\mathcal{O}}}\XS}
\def\Pc{{\ensuremath{\mathcal{P}}}\XS}
\def\Qc{{\ensuremath{\mathcal{Q}}}\XS}
\def\Rc{{\ensuremath{\mathcal{R}}}\XS}
\def\Sc{{\ensuremath{\mathcal{S}}}\XS}
\def\Tc{{\ensuremath{\mathcal{T}}}\XS}
\def\Uc{{\ensuremath{\mathcal{U}}}\XS}
\def\Vc{{\ensuremath{\mathcal{V}}}\XS}
\def\Wc{{\ensuremath{\mathcal{W}}}\XS}
\def\Xc{{\ensuremath{\mathcal{X}}}\XS}
\def\Yc{{\ensuremath{\mathcal{Y}}}\XS}
\def\Zc{{\ensuremath{\mathcal{Z}}}\XS}

% Lettres cursives grasses (majuscules)
%
\def\Acb{{\sbm{\mathcal{A}}}\XS}
\def\Bcb{{\sbm{\mathcal{B}}}\XS}
\def\Ccb{{\sbm{\mathcal{C}}}\XS}
\def\Dcb{{\sbm{\mathcal{D}}}\XS}
\def\Ecb{{\sbm{\mathcal{E}}}\XS}
\def\Fcb{{\sbm{\mathcal{F}}}\XS}
\def\Gcb{{\sbm{\mathcal{G}}}\XS}
\def\Hcb{{\sbm{\mathcal{H}}}\XS}
\def\Icb{{\sbm{\mathcal{I}}}\XS}
\def\Jcb{{\sbm{\mathcal{J}}}\XS}
\def\Kcb{{\sbm{\mathcal{K}}}\XS}
\def\Lcb{{\sbm{\mathcal{L}}}\XS}
\def\Mcb{{\sbm{\mathcal{M}}}\XS}
\def\Ncb{{\sbm{\mathcal{N}}}\XS}
\def\Ocb{{\sbm{\mathcal{O}}}\XS}
\def\Pcb{{\sbm{\mathcal{P}}}\XS}
\def\Qcb{{\sbm{\mathcal{Q}}}\XS}
\def\Rcb{{\sbm{\mathcal{R}}}\XS}
\def\Scb{{\sbm{\mathcal{S}}}\XS}
\def\Tcb{{\sbm{\mathcal{T}}}\XS}
\def\Ucb{{\sbm{\mathcal{U}}}\XS}
\def\Vcb{{\sbm{\mathcal{V}}}\XS}
\def\Wcb{{\sbm{\mathcal{W}}}\XS}
\def\Xcb{{\sbm{\mathcal{X}}}\XS}
\def\Ycb{{\sbm{\mathcal{Y}}}\XS}
\def\Zcb{{\sbm{\mathcal{Z}}}\XS}


% ALPHABET DROIT EN MATHS
% Taille adaptative

\def\AD{{\sdm{A}}\XS}  \def\aD{{\sdm{a}}\XS}
\def\BD{{\sdm{B}}\XS}  \def\bD{{\sdm{b}}\XS}
\def\CD{{\sdm{C}}\XS}  \def\cD{{\sdm{c}}\XS}
\def\DD{{\sdm{D}}\XS}  \def\dD{{\sdm{d}}\XS}
\def\ED{{\sdm{E}}\XS}  \def\eD{{\sdm{e}}\XS}
\def\FD{{\sdm{F}}\XS}  \def\fD{{\sdm{f}}\XS}
\def\GD{{\sdm{G}}\XS}  \def\gD{{\sdm{g}}\XS}
\def\HD{{\sdm{H}}\XS}  \def\hD{{\sdm{h}}\XS}
\def\ID{{\sdm{I}}\XS}  \def\iD{{\sdm{i}}\XS}
\def\JD{{\sdm{J}}\XS}  \def\jD{{\sdm{j}}\XS}
\def\KD{{\sdm{K}}\XS}  \def\kD{{\sdm{k}}\XS}
\def\LD{{\sdm{L}}\XS}  \def\lD{{\sdm{l}}\XS}
\def\MD{{\sdm{M}}\XS}  \def\mD{{\sdm{m}}\XS}
\def\ND{{\sdm{N}}\XS}  \def\nD{{\sdm{n}}\XS}
\def\OD{{\sdm{O}}\XS}  \def\oD{{\sdm{o}}\XS}
\def\PD{{\sdm{P}}\XS}  \def\pD{{\sdm{p}}\XS}
\def\QD{{\sdm{Q}}\XS}  \def\qD{{\sdm{q}}\XS}
\def\RD{{\sdm{R}}\XS}  \def\rD{{\sdm{r}}\XS}
\def\SD{{\sdm{S}}\XS}  \def\sD{{\sdm{s}}\XS}
\def\TD{{\sdm{T}}\XS}  \def\tD{{\sdm{t}}\XS}
\def\UD{{\sdm{U}}\XS}  \def\uD{{\sdm{u}}\XS}
\def\VD{{\sdm{V}}\XS}  \def\vD{{\sdm{D}}\XS}
\def\WD{{\sdm{W}}\XS}  \def\wD{{\sdm{w}}\XS}
\def\XD{{\sdm{X}}\XS}  \def\xD{{\sdm{x}}\XS}
\def\YD{{\sdm{Y}}\XS}  \def\yD{{\sdm{y}}\XS}
\def\ZD{{\sdm{Z}}\XS}  \def\zD{{\sdm{z}}\XS}


% ALPHABET GRAS DROIT
% Permet d'obtenir des caracteres droits directement 
% en mode math ou pas math.
% (Un peu moins utile peut \^eetre)

\def\Av{{\sbv{A}}\XS}  \def\av{{\sbv{a}}\XS}
\def\Bv{{\sbv{B}}\XS}  \def\bv{{\sbv{b}}\XS}
\def\Cv{{\sbv{C}}\XS}  \def\cv{{\sbv{c}}\XS}
\def\Dv{{\sbv{D}}\XS}  \def\dv{{\sbv{d}}\XS}
\def\Ev{{\sbv{E}}\XS}  \def\ev{{\sbv{e}}\XS}
\def\Fv{{\sbv{F}}\XS}  \def\fv{{\sbv{f}}\XS}
\def\Gv{{\sbv{G}}\XS}  \def\gv{{\sbv{g}}\XS}
\def\Hv{{\sbv{H}}\XS}  \def\hv{{\sbv{h}}\XS}
\def\Iv{{\sbv{I}}\XS}  \def\iv{{\sbv{i}}\XS}
\def\Jv{{\sbv{J}}\XS}  \def\jv{{\sbv{j}}\XS}
\def\Kv{{\sbv{K}}\XS}  \def\kv{{\sbv{k}}\XS}
\def\Lv{{\sbv{L}}\XS}  \def\lv{{\sbv{l}}\XS}
\def\Mv{{\sbv{M}}\XS}  \def\mv{{\sbv{m}}\XS}
\def\Nv{{\sbv{N}}\XS}  \def\nv{{\sbv{n}}\XS}
\def\Ov{{\sbv{O}}\XS}  \def\ov{{\sbv{o}}\XS}
\def\Pv{{\sbv{P}}\XS}  \def\pv{{\sbv{p}}\XS}
\def\Qv{{\sbv{Q}}\XS}  \def\qv{{\sbv{q}}\XS}
\def\Rv{{\sbv{R}}\XS}  \def\rv{{\sbv{r}}\XS}
\def\Sv{{\sbv{S}}\XS}  \def\sv{{\sbv{s}}\XS}
\def\Tv{{\sbv{T}}\XS}  \def\tv{{\sbv{t}}\XS}
\def\Uv{{\sbv{U}}\XS}  \def\uv{{\sbv{u}}\XS}
\def\Vv{{\sbv{V}}\XS}  \def\vv{{\sbv{v}}\XS}
\def\Wv{{\sbv{W}}\XS}  \def\wv{{\sbv{w}}\XS}
\def\Xv{{\sbv{X}}\XS}  \def\xv{{\sbv{x}}\XS}
\def\Yv{{\sbv{Y}}\XS}  \def\yv{{\sbv{y}}\XS}
\def\Zv{{\sbv{Z}}\XS}  \def\zv{{\sbv{z}}\XS}
\def\Sigmav{{\sbv{\Sigma}}\XS}

% ALPHABET GREC GRAS 
% Enrichie, completee et modifi\'ee par J.-F. Gio.
% Taille adaptative !

\def\alphab      {{\sbm{\alpha}}\XS}
\def\betab       {{\sbm{\beta}}\XS}
\def\gammab      {{\sbm{\gamma}}\XS}	  \def\Gammab    {{\sbm{\Gamma}}\XS}
\def\deltab      {{\sbm{\delta}}\XS}	  \def\Deltab    {{\sbm{\Delta}}\XS}
\def\epsilonb    {{\sbm{\epsilon}}\XS}
\def\varepsilonb {{\sbm{\varepsilon}}\XS}
\def\etab        {{\sbm{\eta}}\XS}
\def\thetab      {{\sbm{\theta}}\XS}	  \def\Thetab    {{\sbm{\Theta}}\XS}
\def\varthetab   {{\sbm{\vartheta}}\XS}
\def\iotab       {{\sbm{\iota}}\XS}
\def\kappab      {{\sbm{\kappa}}\XS}
\def\lambdab     {{\sbm{\lambda}}\XS}    \def\Lambdab   {{\sbm{\Lambda}}\XS}
\def\mub         {{\sbm{\mu}}\XS}
\def\nub         {{\sbm{\nu}}\XS}
\def\xib         {{\sbm{\xi}}\XS}		  \def\Xib  	  {{\sbm{\Xi}}\XS}
\def\pib         {{\sbm{\pi}}\XS}		  \def\Pib  	  {{\sbm{\Pi}}\XS}
\def\varpib      {{\sbm{\varpi}}\XS}
\def\rhob        {{\sbm{\rho}}\XS}
\def\varrhob     {{\sbm{\varrho}}\XS}
\def\sigmab      {{\sbm{\sigma}}\XS}	  \def\Sigmab    {{\sbm{\Sigma}}\XS}
\def\varsigmab   {{\sbm{\varsigma}}\XS}  \def\Varsigmab {{\sbm{\Varsigma}}\XS}
\def\phib        {{\sbm{\phi}}\XS}  	  \def\Phib 	  {{\sbm{\Phi}}\XS}
\def\varphib     {{\sbm{\varphi}}\XS}
\def\chib        {{\sbm{\chi}}\XS}
\def\psib        {{\sbm{\psi}}\XS}  	  \def\Psib 	  {{\sbm{\Psi}}\XS}
\def\omegab      {{\sbm{\omega}}\XS}	  \def\Omegab    {{\sbm{\Omega}}\XS}
\def\taub        {{\sbm{\tau}}\XS}
\def\upsilonb    {{\sbm{\upsilon}}\XS}   \def\Upsilonb  {{\sbm{\Upsilon}}\XS}
\def\zetab       {{\sbm{\zeta}}\XS}


% CHIFFRES
% Gras, taille adaptative

\def\zerob	 {{\sbv{0}}\XS}
\def\unb		 {{\sbv{1}}\XS}
\def\deuxb	 {{\sbv{2}}\XS}
\def\troisb	 {{\sbv{3}}\XS}
\def\quatreb {{\sbv{4}}\XS}
\def\cinqb	 {{\sbv{5}}\XS}
\def\sixb	 {{\sbv{6}}\XS}
\def\septb	 {{\sbv{7}}\XS}
\def\huitb	 {{\sbv{8}}\XS}
\def\neufb	 {{\sbv{9}}\XS}


% QUELQUES ENSEMBLES
% Taille adaptative

\def\eC{{\ensuremath{\mathbb C}}\XS}
\def\eE{{\ensuremath{\mathbb E}}\XS}
\def\eN{{\ensuremath{\mathbb N}}\XS}
\def\eR{{\ensuremath{\mathbb R}}\XS}
\def\eZ{{\ensuremath{\mathbb Z}}\XS}
\def\eC{{\ensuremath{\mathbb C}}\XS}

